Open Source Software and Data for Human Service Development: A Case Study on Predicting Housing Instability

Open-source data and tools are lauded as essential for replicable and usable social science, though little is known about their use in resource constrained human service provision. This paper examines the challenges and opportunities of open-source tools and data in human service development by using both to forecast failure to pay eviction filings in Bronx County, NY. We use zip code level data from the Housing Data Coalition, the American Community Survey 5-year estimates, and DeepMaps Model of the Labor Force to forecast rates through July 2021. We employ multilevel (MLM) and exponential smoothing (ETS) models using the R project for Statistical Computing, an oft used open-source statistical software. We compare our results to what happened during the same period, to illustrate the efficacy of the open-source tools and techniques employed. We argue open-source data and software may facilitate rapid analysis of public data - a much-needed ability in human service intervention development under increasingly constrained resources - but find public data are limited by the information they reliably capture, limiting their utility by a non-trivial margin of error. The manuscript concludes by considering lessons for human service organizations with limited analytical resources and a vested interest in low-resourced communities.

==> tables/table1.tex <==
% \documentclass[11pt]{article}
\usepackage[margin=1in]{geometry}
\usepackage{booktabs}
\usepackage{threeparttable}

\begin{document}

\begin{table}[htbp]
\centering
\begin{threeparttable}
\caption{Demographics and COVID case rates of Bronx County, New York, and the United States}
\label{tab:demo_covid}
\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{Bronx County, NY} & \multicolumn{2}{c}{United States} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
& N & \% & N & \% \\
\midrule
Total population\tnote{1}                     & 1,435,068 &      & 324,697,795 &      \\
Under 18                                      &   358,404 & 25.0 &  73,429,392 & 22.6 \\
62 and over                                   &   222,687 & 15.5 &  62,456,799 & 19.2 \\
Median household income                       &  \$40,088 &      &   \$62,843  &      \\
\addlinespace
One race                                      & 1,379,200 & 96.1 & 313,933,893 & 96.7 \\
Two or more races                             &    55,868 &  3.9 &  10,763,902 &  3.3 \\
\addlinespace
Hispanic or Latino (any race)                 &   804,018 & 56.0 &  58,479,370 & 18.0 \\
Not Hispanic or Latino                        &   631,050 & 44.0 & 266,218,425 & 82.0 \\
\quad White alone                             &   131,140 &  9.1 & 197,100,373 & 60.7 \\
\quad Black or African American, alone        &   419,473 & 29.2 &  39,977,554 & 12.3 \\
\quad American Indian or Alaska Native, alone &     3,269 &  0.2 &   2,160,378 &  0.7 \\
\quad Asian, alone                            &    51,470 &  3.6 &  17,708,954 &  5.5 \\
\quad Native Hawaiian or Pacific Islander, alone
                                              &       437 &  0.0 &     540,511 &  0.2 \\
\quad Other race, alone                       &     8,971 &  0.6 &     789,047 &  0.2 \\
\addlinespace
Total housing units                           &   529,796 &      & 137,428,986 &      \\
Occupied housing units                        &   503,829 & 95.1 & 120,756,048 & 87.9 \\
Renter-occupied housing units                 &   404,617 & 80.3 &  43,481,667 & 36.0 \\
Average household size, renter-occupied units &       2.72&      &       2.49 &      \\
\addlinespace
Overcrowded ($>$1.5 occupants per room)       &    24,912 &  4.9 &   1,301,261 &  1.1 \\
\addlinespace
Renter households paying 35\% or more of income toward rent\tnote{2}
                                              &   194,258 & 50.5 &  16,328,272 & 40.5 \\
\addlinespace
Civilian labor force 16 years and over, employed
                                              &   601,341 &      & 154,842,185 &      \\
\% employed as share of population            &           & 53.9 &             & 60.0 \\
\addlinespace
With health insurance coverage                & 1,292,952 & 91.4 & 291,458,259 & 91.2 \\
No health insurance coverage                  &   121,071 &  8.6 &  28,248,613 &  8.8 \\
\addlinespace
People with incomes below poverty level       &   392,172 & 28.0 &  42,510,843 & 13.4 \\
People living in deep poverty ($<$50\% of poverty)
                                              &   174,759 & 12.5 &  18,957,462 &  6.0 \\
\addlinespace
Cumulative COVID case rate (per 100,000 people)\tnote{3}
                                              &    10,768 &      &     10,341.3&      \\
Cumulative COVID death rate (per 100,000 people)
                                              &       395 &      &        183.0&      \\
Percent of adult (18+) population with at least one dose of COVID vaccine
                                              &           & 63.3 &             & 68.3 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\footnotesize
\item[1] Demographics from American Community Survey, 2019 5-year estimates.
\item[2] Census could not calculate income-to-housing-cost ratio for all units. The total occupied units used to calculate the percentages are slightly lower than the total occupied units, as follows: Bronx renter-occupied units: 384,296; U.S.\ renter-occupied units: 40,366,338.
\item[3] Bronx COVID data accessed at \texttt{https://www1.nyc.gov/site/doh/covid/covid-19-data.page}. U.S.\ COVID data accessed at \texttt{covid.cdc.gov}. COVID data were downloaded on July 19, 2021.
\end{tablenotes}
\end{threeparttable}
\end{table}

\end{document}
